Networks in a World Unknown: Public WhatsApp Groups in the Venezuelan Refugee Crisis

By early March 2020, five million Venezuelans had fled their home country after its complete economic and institutional collapse, and over 1.6 million have migrated to Colombia. Migrants struggle to start their lives over in Colombia, having arrived with few economic resources, and often no legal documentation, in cities with little to offer them. Venezuelan migrants, however, rely heavily on mobile phones and social media networks as lifelines for information, opportunities, and resources -- making WhatsApp both a critical tool for migrants' settlement and integration, as well as an invaluable source of data through which we can better understand migrant experiences. This thesis explores the dynamics of public WhatsApp groups used by Venezuelan migrants to Colombia, and what they can tell us about how migrants use and share information. We center our research on information spread and trust, especially as they intersect with concentration and geographic heterogeneity within groups. We analyze messages and memberships broadly, then explore interaction within groups, fake news and economic scams, and effects of the coronavirus pandemic. Our results have a range of policy implications, from reflections on Colombia's decision to shut its borders amidst the coronavirus pandemic, to understandings of how aid organizations can effectively share information over social media channels.

==> ch-datamethod/limitations.tex <==
\section{Data Limitations}

While our methodology grants us full access to data from WhatsApp groups, we intentionally limit what data we collect. WhatsApp offers a rich variety of content types for messages, including documents and locations, but many (e.g., documents and locations) are rarely used in our groups of interest, and add unnecessary complexity to both our data collection and analysis.

More significantly, we do not fully download multimedia content (audio recordings, photos, and videos). For photos and videos, we only record a cryptographic hash (only of the thumbnail for videos), and for audio, we only record the duration. To reiterate, our methodology is fully capable of downloading this content (indeed, because our process relies on WhatsApp Web, it ``sees'' exactly what a user would see), but downloading content both involves significant technological burdens and also would require significiant manual analysis to reap benefits (e.g., labeling images and audio).

Moreover, one of the principal researchers in this field has explicitly warned against downloading multimedia content\footnote{Interestingly enough, several of his collaborators have come to center their research on multimedia content in WhatsApp groups. See \cite{resende-misinformation-2019}, \cite{maros-audio-2020}. One has to wonder.}, since some groups are of an adult nature where obscene (and sometimes illegal) content is frequently shared \cite{garimella-whatsapp-2018}.

What this means is that images/videos end up useful in two ways:


==> ch-misinformation/virality.tex <==
\section{Virality of Fake News and Misinformation}

